Research Challenges in Orchestration Synthesis

Contract automata allow to formally define the behaviour of service contracts in terms of service offers and requests, some of which are moreover optional and some of which are necessary. A composition of contracts is said to be in agreement if all service requests are matched by corresponding offers. Whenever a composition of contracts is not in agreement, it can be refined to reach an agreement using the orchestration synthesis algorithm. This algorithm is a variant of the synthesis algorithm used in supervisory control theory and it is based on the fact that optional transitions are controllable, whereas necessary transitions are at most semi-controllable and cannot always be controlled. In fact, the resulting orchestration is such that as much of the behaviour in agreement is maintained. In this paper, we discuss recent developments of the orchestration synthesis algorithm for contract automata. Notably, we present a refined notion of semi-controllability and compare it with the original notion by means of examples. We then discuss the current limits of the orchestration synthesis algorithm and identify a number of research challenges together with a research roadmap.

==> eptcsdata.tex <==
\providecommand{\firstpage}{73}
\providecommand{\publicationstatus}{C. Aubert, C. Di Giusto, S. Fowler \& L. Safina (Eds.):\\
16th Interaction and Concurrency Experience (ICE 2023)\\
EPTCS 383, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.383.5}{10.4204/EPTCS.383.5}}
\pdfoutput=1


==> implementation.tex <==

\begin{minted}[mathescape,fontsize=\scriptsize]{java}
private static <S1> boolean controllabilityPredicate(ModalTransition<S1,Action,State<S1>,CALabel> t,
                                                     ModalTransition<S1,Action,State<S1>,CALabel> tt,
                                                     Set<ModalTransition<S1,Action,State<S1>,CALabel>> str,
                                                     Set<State<S1>> sst){
    return (t.getLabel().getRequester().equals(tt.getLabel().getRequester()))//the same requesting principal
            &&(t.getSource().getState().get(t.getLabel().getRequester())
            .equals(tt.getSource().getState().get(tt.getLabel().getRequester())))//in the same local source state
            &&(tt.getLabel().isRequest()
            &&t.getLabel().getAction().equals(tt.getLabel().getCoAction())||
            tt.getLabel().isMatch()
                    &&t.getLabel().getAction().equals(tt.getLabel().getAction()))//doing the same request
            &&(!reachabilityLazy||
               isReachableWithoutMoving(tt.getSource(),t.getSource(),t.getLabel().getRequester(),str,sst));

}


private static <S1> boolean isReachableWithoutMoving(State<S1> from, State<S1> to,
                                                     Integer principal,
                                                     Set<? extends ModalTransition<S1,Action,State<S1>,CALabel>> str,
                                                     Set<State<S1>> badStates){
    if (from.equals(to)) return true;
    Queue<State<S1>> toVisit = new LinkedList<>(List.of(from));
    Queue<State<S1>> visited = new LinkedList<>();
    while(!toVisit.isEmpty()) {
        State<S1> currentstate = toVisit.remove();
        visited.add(currentstate);
        Set<State<S1>> toAdd = str.parallelStream()
                .filter(x -> x.getSource().equals(currentstate)
                        && x.getLabel().getContent().get(principal) instanceof IdleAction
                        && !visited.contains(x.getTarget())
                        && !badStates.contains(x.getTarget()))
                .map(Transition::getTarget)
                .collect(Collectors.toSet());
        if (toAdd.contains(to))
            return true;
        toVisit.addAll(toAdd);
    }
    return false;
}
 \end{minted}
